Distribution-Free Statistical Dispersion Control for Societal Applications

Explicit finite-sample statistical guarantees on model performance are an important ingredient in responsible machine learning. Previous work has focused mainly on bounding either the expected loss of a predictor or the probability that an individual prediction will incur a loss value in a specified range. However, for many high-stakes applications, it is crucial to understand and control the dispersion of a loss distribution, or the extent to which different members of a population experience unequal effects of algorithmic decisions. We initiate the study of distribution-free control of statistical dispersion measures with societal implications and propose a simple yet flexible framework that allows us to handle a much richer class of statistical functionals beyond previous work. Our methods are verified through experiments in toxic comment detection, medical imaging, and film recommendation.

==> sections/04_method.tex <==


%===========================================================
\section{Distribution-free control of societal dispersion measures} \label{sec:method}

\zhun{add an illustration plot to have an overview of our method}
In this section, we introduce a simple yet general framework to control the nonlinear structures in statistical dispersion measures discussed in the previous section and  obtain rigorous upper bounds on these quantities. We will only provide a high-level summary of important concepts in our framework in Section~\ref{sec:control} and leave detailed derivations and examples to the appendix. In this section, our discussion will focus on quantities related to the inverse of CDFs, but similar results could be obtained for CDFs. To describe our framework, we will make use of the following definitions/properties. 

%Let us use $\mathscr{L}(\bR)$ to denote the family of functions that maps $\bR$ to $\bR$. 
For two functions $G, H: \bR \rightarrow \bR$, we say $G \succeq H$ if $G(x) \ge H(x)$ for all $x \in \mathbb{R}$. Similarly, we denote $G\preceq H$ if $G(x) \le H(x)$.
%Let us use $\mathscr{L}(\bR)$ to denote the family of functions that maps $\bR$ to $\bR$. For two functions $G$ and $H$ in $\mathscr{L}(\bR)$, we say $G \succeq H$ if $G(x) \ge H(x)$ for all $x \in \mathbb{R}$ and we say a transformation $\phi$ that maps a function $G\in\mathscr{L}(\bR)$ to another function $H\in\mathscr{L}(\bR)$ increasing (or decreasing) if $\phi\circ G \succeq \phi\circ H$ (or $\phi\circ H \succeq \phi\circ G$). For example, $\phi\circ F=F^-$ is a decreasing transformation.
\zhun{remove this}
\begin{proposition}\label{prop:flip}
For the CDF $F$ of $X$, if there exists two increasing functions $F_U,F_L$ such that $F_U \succeq F \succeq F_L$, then we have $F^-_L \succeq F^- \succeq F^-_U$.
\end{proposition}

%RZ: cutting this out as it is redundant with the earlier footnote.
%\textbf{Distribution-free guarantee.} The last thing we want to emphasize before our analysis is about the ``distribution-free" nature of our guarantees. This should be viewed as being over $(Z,Y)_{1:n}$ instead of $X_{1:n}$, since if we recall $X=\ell(h(Z),Y)$, $\ell$ is known to us, which means we can fully exploit the properties of $\ell$. For instance, in \citep{angelopoulos2021learn}, the loss used in false discovery rate (FDR) control is always bounded between $0$ and $1$. %If in some cases, the boundedness assumption of $(Z,Y)_{1:n}$ is imposed (e.g. we have some prior knowledge about $Z,Y$, such as $Y$ is binary), we still consider this condition mild and say the guarantee obtained is ``almost distribution-free''. 











%========================================
\subsection{Control of nonlinear functions of CDFs}\label{sec:nonlinear}\label{sec:control}





We start with bounding $\xi(F^-)$, which maps $F^-$ to another function of $\bR$. We use $(\hat{F}^\delta_{n,L},\hat{F}^\delta_{n,U})$ to denote a $(1-\delta)$-confidence bound pair ($(1-\delta)$-CBP), which satisfies $\bP(\hat{F}^{\delta}_{n,U}\succeq F\succeq \hat{F}^{\delta}_{n,L})\ge 1-\delta$. We defer the details about methods to obtain  $(1-\delta)$-CBP to Section~\ref{sec:two-side}.

%When there is only one-sided bound considered, we also abuse the notation and denote $\hat{F}^{\delta}_{n,U}$ as a $(1-\delta)$-upper bound confidence ($(1-\delta)$-CDF-UBC) function of $F$ constructed by $X_{1:n}$, which satisfies $\bP(\hat{F}^{\delta}_{n,U}\succeq F)\ge 1-\delta$. Similarly, we denote $\hat{F}^{\delta}_{n,L}$ as a $(1-\delta)$-lower bound confidence ($(1-\delta)$-CDF-LBC) function of $F$ constructed by $X_{1:n}$, which satisfies $\bP(F\succeq \hat{F}^{\delta}_{n,L})\ge 1-\delta$. We defer the details about methods to obtain  $(1-\delta)$-CDF-CBP to Section~\ref{sec:two-side}. We will only discuss functions of the inversed CDFs in our derivation, but similar results could be obtained for CDFs. We denote the corresponding inversed CDFs as $(\hat{F}^{\delta,-}_{n,L},\hat{F}^{\delta,-}_{n,U})$.
\zhun{write out specific examples for each of them, and add theorem environment}
\paragraph{Control for a monotonic function.} We start with the simplest case where $\xi$ is a monotonic function in the range of $X$. For example, if $\xi$ is an increasing function, by Proposition~\ref{prop:flip}, we have $\xi(\hat{F}^{\delta,-}_{n,L})\succeq \xi(\hat{F}^{-}) \succeq  \xi(\hat{F}^{\delta,-}_{n,U})$ holds with probability at least $1-\delta$. This could be applied to provide bounds for Gini coefficient and Atkinson index by controlling the numerator and denominator separately as integrals of monotonic functions of $F^-$.

\paragraph{Control for absolute and polynomial functions.} Many of our exemplified societal dispersion measures involve absolute-value functions 
% (e.g., the Hoover index in the appendix involves $|F^--\bE[X]|$).
, e.g. the Hoover index in the appendix or maximum group differences.
 More generally, how can we tackle polynomial functions of inverse CDFs, such as in the CDFs of extreme observations? It is not hard to notice that  if $s_L\le s\le s_U$, then $$s_L\bm{1}\{s_L\ge 0\}-s_U\bm{1}\{s_U\le 0\}\le |s|\le \max\{|s_U|,|s_L|\}.$$ Thus, for $|F^-|$, we can plug in $\hat{F}^{\delta,-}_{n,L}$ and $\hat{F}^{\delta,-}_{n,U}$ to replace $s_U$ and $s_L$ to obtain two-sided bounds. More generally, for any polynomial function $\phi(s)=\sum_{k=0}\alpha_k s^k$, if $k$ is odd, $s^k$ is monotonic w.r.t. $s$; if $k$ is even, $s^k=|s|^k$. Thus, we can group $\alpha_k s^k$ according to the sign of $\alpha_k$ and whether $k$ is even or odd, and flexibly use the upper and lower bounds for the absolute value function and monotonic functions to obtain an overall upper bound. 

\paragraph{Control for a general function.} Recall that \citet{berkhouch2019spectral} studies forms like $$\int_{0}^1\xi(F^-(\alpha))\psi(\alpha)d\alpha$$ to quantify how sensitive the $\alpha$-VaR value is w.r.t its parameter $\alpha$. For nonlinear functions beyond polynomials, consider the example where $\xi = e^x+e^{-x}$. This can be readily bounded since it is a mixture of monotone functions.
%highlight $\alpha$-VaR with small or large $\alpha$. 
%Notice the above function is a mixture of monotonic functions, which is easy to tackle. 
To handle general nonlinearities, we introduce the class of functions of bounded total variation. Roughly speaking, a function of bounded total variation on an interval means that it wiggles boundedly on that interval. It is a very rich class including all continuously differentiable or Lipchitz continuous functions. The following theorem shows that such functions can always be decomposed into two monotonic functions. 

\begin{theorem}\label{thm:1}
For $(\hat{F}^\delta_{n,L},\hat{F}^\delta_{n,U})$, if $\xi$ is a function with bounded total variation on the range of $X$, there exists increasing functions $f_1,f_2$ with explicit and calculable forms, such that with probability at least $1-\delta$,
$\xi(F^-)\preceq f_1(\hat{F}^{\delta,-}_{n,L})-f_2(\hat{F}^{\delta,-}_{n,U}).$
\end{theorem}

%We establish that with the following informal theorem. Please refer to the appendix for the formal one.
%\begin{theorem}[\textbf{Informal}]
%For $(\hat{F}^\delta_{n,L},\hat{F}^\delta_{n,U})$, if $\xi$ is a function with bounded total variation on the range of $X$, there exist two increasing functions $f_1,f_2$ with explicit and calculable forms, such that with probability at least $1-\delta$,
%$\xi(F^-)\preceq f_1(\hat{F}^{\delta,-}_{n,L})-f_2(\hat{F}^{\delta,-}_{n,U}).$
%\end{theorem}








%========================================
\subsection{Control of nonlinear functionals of CDFs and beyond}\label{sec:beyond}
Finally, we show how our techniques from the previous section can be applied to handle the general form: $\int_{0}^1\xi(T(F^-(\alpha)))\psi(\alpha)d\alpha$ %\psi(p) \xi(T(F^-(p))dp$ 
where $\psi$ can be a general function (not necessarily non-negative),  $\xi$ can be a {\it functional} of the inverse CDF. 
%function $\psi$ that not necessarily to be non-negative, 
%It is straightforward to apply the techniques in Section~\ref{sec:control} to provide upper bounds. 
To handle $\xi(T(F^-))$, we can first obtain two-sided bounds for $T(F^-)$ if $T(F^-)$ is in the class of QBRMs or in the form of $\int \psi(p) \xi_2(F^-(p))dp$ for some nonlinear function $\xi_2$
(as in \citet{berkhouch2019spectral}).
%f the form previously mentioned. 
We can also generalize the weight functions in QBRMs from non-negative ones to  general weight functions immediately once we notice that $\psi$ can be decomposed into two non-negative functions, i.e. $\psi=\max\{\psi,0\}-\max\{-\psi,0\}$. Then, we can provide upper bounds for terms like $\int \max\{\psi,0\} \xi(F^-(p))dp$ by adopting an upper bound for $\xi(F^-)$. 

%\TP{Zhun -- this section 4.2 overlaps quite a bit with the previous subsection = "Control for a general function". Can you merge 4.2 with the above? I think this can be shortened to just one or two sentences discussing how to adapt above to handle more general weight functions. Also I went back to theorem form which Rich and I prefer. I think Rich just didn't like the word "Informal"}


%========================================
%\subsection{Control of nonlinear functions of functionals of (the inverse of) CDFs}










%========================================
%\subsection{Calculation of some societal statistical dispersion examples }





%========================================
\subsection{Methods to obtain confidence two-sided bounds for CDFs}\label{sec:two-side}
Now, we formally discuss how to provide $(1-\delta)$-CBP bounds. %(\hat{F}^\delta_{n,L},\hat{F}^\delta_{n,U})$.
For $\{X_i\}_{i=1}^n$, let $X_{(1)} \le \ldots \le X_{(n)}$ denote the corresponding order statistics. For the uniform distribution over [0,1], i.e. $\cU(0, 1)$, let $U_1, \ldots, U_n \sim^{iid} \cU(0, 1)$ denote the corresponding order statistics $U_{(1)} \le \ldots \le U_{(n)}$.



We extend the techniques developed in \citet{snell2022quantile},
which
%In \citep{snell2022quantile}, the authors mainly discuss how to obtain $\hat{F}^\delta_{n,L}$. Their technique 
produces one-sided (lower) confidence bounds on the uniform order statistics, and uses these to bound $F$ by considering a one-sided minimum goodness-of-fit (GoF) statistic of the following form: $S := \min_{1 \le i \le n} s_i(U_{(i)}),$ where $s_1, \ldots,s_n : [0,1] \rightarrow \mathbb{R}$ are right continuous monotone nondecreasing functions. Thus,
$\bP(\forall i: F(X_{(i)}) \ge s_i^{-}(s_\delta)) \ge 1-\delta,$
for $s_\delta=\inf_r\{r: \bP(S\ge r)\ge 1-\delta\}$. Based on that, it is easy to construct $\hat{F}^\delta_{n,L}$ with conservative completion of the CDF. %(see \citep{snell2022quantile}). 
They found that by choosing appropriate $s_i$'s,
via Berk-Jones bounds, the construction of $\hat{F}^\delta_{n,L}$ is typically tighter than the Dvoretzky–Kiefer–Wolfowitz (DKW) inequality.


\subsubsection{A reduction approach to constructing upper bounds of CDFs}\label{sec:reduction}

%Here, we further show that a simple transformation of $\{s_i^{-}(s_\delta)\}_{i=1}^n$ can immediately yield upper bounds for $F(X_{(i)})$'s, which further be used to obtain $\hat{F}^\delta_{n,U}$ with conservative completion of the CDF. 
Now we show how we can leverage this approach to produce two-sided bounds. In the following lemma we show how a CDF upper bound can be reduced to constructing lower bounds. %under a transformation.
\zhun{add explanation to the $1-\delta$ inflation question}
\begin{lemma}\label{lemma:two-sided}
For $0\le L_1\le L_2\cdots\le L_n\le 1$, if $\bP(\forall i: F(X_{(i)}) \ge L_i) \ge 1-\delta,$
then, we have 
$$\bP(\forall i: \lim_{\epsilon\rightarrow 0^+}F(X_{(i)}-\epsilon) \le 1-L_{n-i+1}) \ge 1-\delta.$$
Furthermore, let $R(x)$ be defined as $1-L_{n}$ if $x<X_{(1)}$; $1-L_{n-i+1}$ if $X_{(i)}\le x<X_{(i+1)}$ for $i\in\{1,2,\cdots,n-1\}$; $1$ if $X_{(n)}\le x$. Then, $F\preceq R$.
\end{lemma}
Thus, we can simultaneously obtain $(\hat{F}^\delta_{n,L},\hat{F}^\delta_{n,U})$ by setting $L_i=s^-_i(s_\delta)$ and applying (different) CDF conservative completions. All the bounds in \citet{snell2022quantile} can be applied directly to our framework.






















% \begin{figure}[!ht]
% \centering
%     \includegraphics[width=\textwidth]{figures/fuq_figure_2.png}
%     \caption{Example illustrating the construction of distribution-free CDF lower and upper bounds by bounding order statistics.  On the left, order statistics are drawn from a uniform distribution.  On the right, samples are drawn from a real loss distribution, and the corresponding Berk-Jones CDF lower and upper bound are shown in black.  Our distribution-free method gives bound $b^{(l)}_i$ and $b^{(u)}_i$ on each sorted order statistic such that the bound depends only on $i$, as illustrated in the plots for $i=7$ (shown in orange). On the left, 1000 realizations of $U_{(1)}, \ldots, U_{(n)}$ are shown in blue.  On the right, 1000 empirical CDFs are shown in blue, and the true CDF $F$ is shown in red.}
%     \label{fig:synthetic}
% \end{figure}



\subsubsection{Numerical optimization towards tighter bounds for statistical functionals} \label{sec:num}
One drawback of the QBRM bounding approach
%framework of \citep{snell2022quantile} 
is that it is not weight function aware:  when controlling $\int_0^1\psi(p)F^-(p)dp$ for a non-negative weight function $\psi$, the procedure ignores the structure of $\psi$, as it first obtains $\hat{F}^\delta_{n,L}$, then provides an upper bound $\int_0^1\psi(p)\hat{F}^{\delta,-}_{n,L}(p)dp$.  
%Although they further provide two tailored truncated Berk-Jones bounds for CVaR and VaR interval, that is far from a general approach. 
This motivates %us to provide 
the following numerical optimization method, which shows significant improvement over previous bounds including DKW and Berk-Jones bounds. The key observation is that for any $0\le L_1\le\cdots\le L_n\le 1$, we have $\bP\big(\forall i,~ F(X_{(i)})\ge L_i\big)\ge n!\int^1_{L_n}dx_n\int^{x_{n}}_{L_{n-1}}dx_{n-1}\cdots\int^{x_{2}}_{L_{1}}dx_{1},$ where the right-hand side integral is a function of $\{L_i\}_{i=1}^n$ and its partial derivatives can be calculated by the package in \citet{moscovich2016exact} exactly.
%\begin{align*}
%\bP\big(\forall i,~ F(X_{(i)})\ge L_i\big)\ge n!\int^1_{L_n}dx_n\int^{x_{n}}_{L_{n-1}}dx_{n-1}\cdots\int^{x_{2}}_{L_{1}}dx_{1}.
%\end{align*}

Consider controlling $\int_0^1\psi(p)F^-(p)dp$ as an example. For any $\{L_i\}_{i=1}^n$ satisfying $$\bP\big(\forall i,~ F(X_{(i)})\ge L_i\big)\ge 1-\delta,$$ one can use conservative CDF completion to obtain $\hat{F}^{\delta}_{n,L}$, i.e. 
$$\int_0^1\psi(p)\xi(\hat{F}^{\delta,-}_{n,L}(p))dp= \sum_{i=1}^{n+1}\xi(X_{(i)})\int_{L_{i-1}}^{L_{i}}\psi(p)dp,$$ where $L_{n+1}$ is $1$, $L_0=0$, and $X_{(n+1)}=\infty$ or a known upper bound for $X$. Then, we can formulate tightening the upper bound as an optimization problem:
\vspace{0.1in}
$$\min_{\{L_i\}_{i=1}^n}\sum_{i=1}^{n+1}\xi(X_{(i)})\int_{L_{i-1}}^{L_{i}}\psi(p)dp$$
such that
$\bP\big(\forall i,~ F(X_{(i)})\ge L_i\big)\ge 1-\delta,~ \text{and}~0\le L_1\le \cdots\le L_n\le 1.$
We optimize the above problem with %surrogates and 
gradient descent and a simple post-processing procedure to make sure the obtained $\{\hat L_i\}_{i=1}^n$ strictly satisfy the above constraints. 
%However, $\{\hat L_i\}_{i=1}^n$ may not satisfy the above constraints since we use surrogates. In order to obtain $L_i$'s strictly satisfy the constraints, we further do post-processing to find an adjustment $\gamma^*\in[0,\min_i \hat L_i]$ such that $\gamma^*=\inf \{\gamma:\bP\big(\forall i,~ F(X_{(i)})\ge \hat{L}_i-\gamma\big)\ge 1-\delta\},$ which could be solved by binary search given the monotonicity w.r.t $\lambda$. 
In practice, we re-parameterize $\{L_i\}_{i=1}^n$ with a network $\phi_\theta$ that maps $n$ random seeds to a function of the $L_i$'s, and transform the optimization objective from $\{L_i\}_{i=1}^n$ to $\theta$. 
We find that a simple parameterized neural network model with 3 fully-connected hidden layers of dimension 64 is enough for good performance and robust to hyper-parameter settings. 

\zhun{add back post-processing procedure}
 

==> sections/05_bounds.tex <==
\newpage
%========================================
\section{Methods to obtain confidence bounds for (the inverse of) CDFs}





\subsection{A reduction approach to constructing upper bounds of CDFs}\label{sec:reduction}

\begin{figure}[!ht]
\centering
    \includegraphics[width=\textwidth]{figures/fuq_figure_2.png}
    \caption{Example illustrating the construction of distribution-free CDF lower and upper bounds by bounding order statistics.  On the left, order statistics are drawn from a uniform distribution.  On the right, samples are drawn from a real loss distribution, and the corresponding Berk-Jones CDF lower and upper bound are shown in black.  Our distribution-free method gives bound $b^{(l)}_i$ and $b^{(u)}_i$ on each sorted order statistic such that the bound depends only on $i$, as illustrated in the plots for $i=7$ (shown in orange). On the left, 1000 realizations of $U_{(1)}, \ldots, U_{(n)}$ are shown in blue.  On the right, 1000 empirical CDFs are shown in blue, and the true CDF $F$ is shown in red.}
    \label{fig:synthetic}
\end{figure}



\subsection{Numerical optimization towards tighter bounds for statistical functionals}


==> sections/07_extension.tex <==
%===========================================================
\section{Extension}
\zhun{1. multi-dim CDF control example Gini correlation 2. multi-dim quantile definition and bounds}

